Mixture Content Selection for Diverse Sequence Generation

Generating diverse sequences is important in many NLP applications such as question generation or summarization that exhibit semantically one-to-many relationships between source and the target sequences. We present a method to explicitly separate diversification from generation using a general plug-and-play module (called SELECTOR) that wraps around and guides an existing encoder-decoder model. The diversification stage uses a mixture of experts to sample different binary masks on the source sequence for diverse content selection. The generation stage uses a standard encoder-decoder model given each selected content from the source sequence. Due to the non-differentiable nature of discrete sampling and the lack of ground truth labels for binary mask, we leverage a proxy for ground truth mask and adopt stochastic hard-EM for training. In question generation (SQuAD) and abstractive summarization (CNN-DM), our method demonstrates significant improvements in accuracy, diversity and training efficiency, including state-of-the-art top-1 accuracy in both datasets, 6% gain in top-5 accuracy, and 3.7 times faster training over a state of the art model. Our code is publicly available at https://github.com/clovaai/FocusSeq2Seq.

==> 05-results-t-qg-human.tex <==
\begin{table}[!h]
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l||ccc||ccc}
        \hline
         & \multicolumn{3}{c||}{Diversity (\%)} & \multicolumn{3}{c}{Accuracy (\%)} \\
        \hline
        \multicolumn{1}{c||}{Baselines} & Win & Lose & Tie & Win & Lose & Tie \\
        vs. 3-D. Beam & \textbf{49.7} & 31.3 & 19.0 & \textbf{43.9} & 36.9 & 19.2 \\
        vs. 3-T. Sampling & \textbf{46.7} & 35.1 & 18.2 & \textbf{45.3} & 36.1 & 18.6 \\
        vs. 3-M. Decoder & \textbf{47.6} & 32.5 & 19.9 & \textbf{41.8} & 36.0 & 22.2 \\
        \hline
    \end{tabular}
    }
    \caption{
    Human evaluation on SQuAD question generation.
    }
    \label{table:human_qg}
\end{table}

==> 05-results-t-sm-human.tex <==
\begin{table}[!h]
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l||ccc||ccc}
        \hline
         & \multicolumn{3}{c||}{Diversity (\%)} & \multicolumn{3}{c}{Accuracy (\%)} \\
        \hline
        \multicolumn{1}{c||}{Baselines} & Win & Lose & Tie & Win & Lose & Tie \\
        vs. 3-D. Beam & \textbf{50.4} & 40.9 & 8.7 & \textbf{46.2} & 38.5 & 15.3 \\
        vs. 3-T. Sampling & \textbf{48.7} & 42.0 & 9.3 & \textbf{50.3} & 41.2 & 8.5 \\
        vs. 3-M. Decoder & \textbf{49.7} & 39.6 & 10.7 & \textbf{46.5} & 37.5 & 16.0 \\
        \hline
    \end{tabular}
    }
    \caption{
    Human evaluation on CNN-DM abstract summarization.
    }
    \label{table:human_sm}
\end{table}
